A Cryptographic Test of Quantumness and Certifiable Randomness from a Single Quantum Device

We consider a new model for the testing of untrusted quantum devices, consisting of a single polynomial-time bounded quantum device interacting with a classical polynomial-time verifier. In this model we propose solutions to two tasks - a protocol for efficient classical verification that the untrusted device is "truly quantum," and a protocol for producing certifiable randomness from a single untrusted quantum device. Our solution relies on the existence of a new cryptographic primitive for constraining the power of an untrusted quantum device: post-quantum secure trapdoor claw-free functions which must satisfy an adaptive hardcore bit property. We show how to construct this primitive based on the hardness of the learning with errors (LWE) problem.

==> introduction.tex <==



In this paper we propose solutions to two basic tasks: how to generate \emph{certifiably random} strings from a \emph{single untrusted} quantum device (also referred to as a prover), and how to efficiently verify that an untrusted device is ``truly" quantum, as opposed to classical. %, behavior.  
The setting we consider is 
one where the quantum device is polynomial-time bounded but untrusted, and the verifier is entirely classical and also polynomial-time bounded. The peculiarity of this setting is that it allows the verifier to leverage post-quantum cryptography, i.e. the existence of cryptographic primitives that can be implemented efficiently on a classical computer but that cannot be broken by any efficient quantum computer. 

There has been considerable research into certifiable random number expansion from quantum devices~\cite{Colbeck09,Pironio,VV12,miller2016robust,arnon2018practical}, including experimental demonstrations~\cite{bierhorst2018experimentally}. However, all prior works providing verifiable guarantees have focused on the setting where there are multiple quantum devices
that share entanglement, and where the randomness certification relies on the violation of a Bell inequality. More generally, the violation of Bell inequalities provides a powerful technique for the classical testing of quantum devices --- the obvious downside being that it is limited to situations with multiple non-communicating quantum devices that share entanglement. Here we propose a new setting for classical testing, where bounds on the computational power of a single quantum device are leveraged by a classical verifier. 

Specifically, in the context of certifiable random number expansion, we consider the following model. Given a security parameter as input, an all-powerful adversary is tasked to provide (i) a computationally efficient device (concretely, a family of polynomial-size quantum circuits) and (ii) a bipartite quantum state $\rho_{\reg{DE}}$ such that the register $\reg{D}$ has polynomially many qubits and $\reg{E}$ may be unbounded. The protocol is then executed between a trusted verifier and the device, whose initial state is provided by register $\reg{D}$. The computational assumption that we make is that the device is unable to break the post-quantum cryptographic assumption during the execution of the protocol. Under this assumption, the guarantee that we obtain is that the output 
of the protocol is statistically indistinguishable from a uniformly random sequence of bits, from the point of view of the \emph{computationally unbounded} adversary that initially designed the device and has access to the state in register $\reg{E}$ on which it may perform an arbitrary measurement. 

This information-theoretic guarantee is identical to that offered in the aforementioned works~\cite{VV12,miller2016robust,arnon2018practical}. The guarantee is stronger than computational pseudorandomness (that is easily achievable under standard cryptographic assumptions, since the verifier starts with a short uniformly random seed). Indeed, for the case of computational pseudorandomness once the outcome has been produced it is always possible (with sufficiently large computational power) to design a statistical test that will distinguish the real outcome from a truly uniform string. In the case of our scheme this is not possible: as long as the device is efficient for the duration of the protocol, the outcome is indistinguishable from uniform at all later times.\footnote{In quantum cryptography this form of security is sometimes referred to as \emph{everlasting security}.}


%It is the same guarantee as that offered in the aforementioned works; the difference is that, instead of relying on spatial isolation of two quantum devices during the protocol, we rely on the computational boundedness of a single quantum device during the protocol. 

The specific cryptographic primitive we rely on is the existence of a post-quantum secure trapdoor claw-free  (in short, TCF) family of functions $f:\{0,1\}^n \rightarrow \{0,1\}^m$, the post-quantum analogue of a notion introduced by Goldwasser, Micali and Rivest in the context of digital signatures \cite{GoldwasserMR84}.
A TCF is a $2$-to-$1$ function $f$ that satisfies the following properties: $f(x)$ is efficiently computable on a classical computer, and if $f(x) = y$, then there is a unique 
$x' \neq x$ such that $ f(x') = y$. Moreover, with knowledge of a secret trapdoor  it is possible to efficiently (classically) compute $x$ and $x'$ from $y$, but without the trapdoor there is no efficient 
quantum algorithm that can compute such a claw, a triple $(x, x', y)$, for any $y$.

By contrast, a quantum algorithm can simultaneously hold an image $y$, as well as a superposition $\frac{1}{\sqrt{2}}(\ket{x} +\ket{x'})$ over two preimages of $y$, simply by 
evaluating $f$ on a uniform superposition over all inputs and measuring the image $y$. At this point, measuring the quantum state in the standard basis will yield a random preimage, $x$ or $x'$. This is not any stronger than a classical device could do, by first sampling a random $x$ and then computing $y=f(x)$. However, the quantum device can do something different from directly measuring a preimage. Instead, the device can perform Fourier sampling (Hadamard transform followed by a measurement), which yields a random $n$-bit string $d$ such that $d\cdot(x \oplus x') = 0$, thereby revealing some joint information about \emph{both} preimages of $y$. From the point of view of the classical verifier a device that performs these tasks is modeled as an untrusted black box that outputs $y$, and then either a string $x$ or a string $d$. Assuming the verifier knows the secret trapdoor, given $y$ she can efficiently compute both preimages  $x$ and $x'$ and verify that indeed $d\cdot(x \oplus x') = 0$. At a high level, the consideration of a cryptographic primitive equipped with a trapdoor restores some symmetry between the quantum prover (the untrusted quantum device) and the classical verifier, by providing a primitive which allows the quantum capabilities of the prover
to play a useful role while at the same time giving the classical verifier a handle, namely the ability to compute both $x$ and $x'$, that the prover does not have access to. 

\paragraph{A test of quantumness.}
We refer to the protocol that consists of first, requesting a value $y$ in the range of $f$, and then, executing either the preimage test (receive a string $x$ and check that $f(x)=y$), or the equation test (receive a string $d$ and check, using the trapdoor, that $d\cdot (x\oplus x')=0$, where $x,x'$ are the two preimages of $y$), each chosen with probability $\frac{1}{2}$, as the \emph{single round test}.

The ability to succeed in the single round test seems to be a unique quantum capability. To argue that no classical procedure could succeed in the test, we describe a TCF construction based on the learning with errors problem (LWE) that has additional security guarantees, most notably the ``adaptive hardcore bit'' property that is explained below. 
%This condition helps in going beyond the analysis of a single round of our randomness-generation protocol (this analysis can be performed based on a more generic requirement for the TCF) to guarantee randomness accumulation across multiple rounds, a more stringent requirement. 
For clarity, in this paper we refer to the specific kind of TCF that we rely on as an NTCF, or post-quantum secure noisy trapdoor claw-free family. We give a construction of an NTCF that rests on the hardness of the Learning with Errors (LWE) problem, introduced by Regev \cite{regev2005}, with slightly super-polynomial noise ratio, against quantum polynomial-time attacks with nonuniform quantum advice  (for which the state of the art classical and quantum attacks scale exponentially with the dimension).  This construction is similar to the one used in \cite{mahadev2017classicalv1}, albeit with some changes in parameters that allows us to prove the following crucial adaptive hardcore bit property: roughly, that given the public parameters of the NTCF it is computationally intractable to sample from any distribution on quadruples $(y, x, d, b)$ such that both conditions $f(x) = y$ and $b = d\cdot (x\oplus x')$ hold with probability non-negligibly larger than $\frac{1}{2}$. Very informally, this says that the condition that no efficient quantum algorithm can exhibit a claw $(x, x', y)$ for the NTCF
can be greatly strengthened to assert that no efficient quantum algorithm can even exhibit $(x, y)$ and a nontrivial advantage in guessing any generalized bit of $x'$ of its choice --- where a generalized bit is $d \cdot x'$ for any choice of $d$. Note that this is much stronger than a standard hardcore bit, which would assert intractability only for fixed $d$. 


%that given the public parameters of the NTCF it is computationally intractable to sample from any distribution on quadruples $(y, x, d, b)$ such that both conditions $f(x) = y$ and $b = d\cdot (x\oplus x')$ hold with probability non-negligibly larger than $\frac{1}{2}$.

Assuming such an adaptive hardcore bit property, it is possible to show that passing the single round test constitutes a proof of quantumness of the device. This is because any efficient classical algorithm that can reliably succeed in both the preimage test and the equation test could be ``rewound'' to simultaneously answer both challenges, thus contradicting the adaptive hardcore bit property. 

This result has implications for an important milestone in the experimental realization of quantum computers, namely ``quantum supremacy'': a proof that an (untrusted) quantum computing device performs some computational task that cannot be solved classically without impractical resources. While this could in principle be achieved by demonstrating quantum factoring, the latter requires quantum resources well beyond the capability of near term experiments. Instead current proposals are based on sampling problems (see e.g.~\cite{harrow2017quantum} for a recent survey). The major challenge for these proposals is verifying that the quantum computer did indeed sample from the desired probability distribution, and all existing proposals rely on exponential time classical algorithms for verification. By contrast, our single round test provides a proof of quantumness that can be verified by a classical verifier in polynomial time. This proposal seems promising from a practical viewpoint --- indeed, even using off-the-shelf bounds for  LWE-based cryptography suggests that a protocol providing $50$ bits of security could be implemented with a quantum device of around $2000$ qubits (see e.g.~\cite{lindner2011better}). It would  be worth exploring whether there are clever implementations of this scheme that can lead to a protocol in the $200-500$ qubit range. Our protocol is robust to a device that only successfully answers the verifier's challenges with a sufficiently large, but constant, success probability; it would be interesting to explore whether such a device could be implemented without resorting to general fault-tolerance techniques.


\paragraph{Certifiable randomness.}

The challenge in achieving certifiable randomness lies in using computational assumptions to establish not pseudorandomness, but rather that the output of the protocol must be (close to) statistically random. The goal of the protocol we sketch below is to leverage the properties of the NTCF to characterize the quantum state and measurements of the untrusted quantum device --- essentially showing that it must have a qubit initialized in state $\ket{+}$, which it measured in the standard basis, thus generating statistical randomness. This is the analogue of the use of the violation of Bell inequalities to characterize the state of the device in entanglement-based testing. \unote{}

We first explain how to show a device that succeeds in the single round test must generate randomness. In the test the device must make one of two measurements: either a ``preimage'' measurement, or an ``equation'' measurement. We focus on a single bit of information provided by each measurement. The ``preimage'' measurement can be treated as a projection into one of two orthogonal subspaces corresponding to the two preimages $x,x'$ for the element $y$ that the device has returned to the verifier. The ``equation'' measurement can similarly be coarse-grained into a projection on one of two orthogonal subspaces, ``valid'' or ``invalid'', i.e.\ the subspace that corresponds to all measurement outcomes $d$ such that $d\cdot(x \oplus x') = 0$, or the subspace associated with outcomes $d$ such that $d\cdot(x \oplus x') = 1$. 

Applying Jordan's lemma, it is possible to decompose the device's Hilbert space into a direct sum of one- and two-dimensional subspaces, such that within each two-dimensional subspace the ``preimage'' and ``equation'' measurements each correspond to an orthonormal basis, such that the two bases make a certain angle with each other. We argue that almost all angles must be very close to $\pi/4$. Indeed, whenever the angles are \emph{not} near-maximally unbiased, it is possible to show that by considering the effect of performing the measurements in sequence, one can devise an ``attack'' on the NTCF of a kind that contradicts the adaptive hardcore bit property of the NTCF --- informally, the attack can simultaneously produce a valid preimage and a valid equation, with non-negligible advantage. 

As a result it is possible to show that the state and (coarse-grained)
measurements of the device are, up to a global change of basis, close to the following: the device starts with a qubit initialized to $\ket{+}$, which it measures in the standard basis for the case of a preimage test and in the Hadamard basis for the case of an equation test. The fact that an efficient quantum device cannot break the cryptographic assumption has thus been translated into a characterization of the state and actions of the quantum device, which 
further implies that the output of the device in the single round test must contain close to a bit of true (information theoretic) randomness. 

One might further conjecture that for a generic TCF  (e.g.\ modeled as a random oracle), if the output of any efficient quantum device passes the single round test with non-negligible advantage over $\frac{1}{2}$, then the pair $y,d$ returned in the equation test must have high min-entropy. Such a strong statement would immediately yield a randomness certification protocol. Among the many difficulties in showing such a statement is that both $y$ and $d$ may be adaptively and adversarially chosen --- in the single round protocol above this issue is addressed by the adaptive hardcore bit property of the NTCF. 
%While we do not know how to prove this, we are still able to design and analyze a simple protocol, that can be based on any TCF family with suitable cryptographic properties, and succeeds in certifiable randomness expansion from a single untrusted quantum (polynomial-time) device. 


\paragraph{Outline of randomness generation protocol.}
Going beyond the analysis of the single round test requires significantly more work. So far we have argued that if an efficient quantum algorithm has the ability to generate a valid equation with probability sufficiently close to $1$, then, if instead it is asked for a preimage, this preimage must be close to uniformly distributed over the two possibilities. To leverage this our randomness expansion protocol proceeds in multiple rounds, repeatedly asking for new images $y$ and a preimage of $y$ (to generate randomness) while inserting a few randomly located equation tests to test the device. Each time an ``equation'' challenge has been answered, we refresh the pseudorandom keys used for the NTCF. This is required to avoid a simple ``attack'' by the device, which would repeatedly use the same $y$, preimage $x$, and guessed equation $d$ --- succeeding in the protocol with probability $\frac{1}{2}$ without generating any randomness. 

Let's call the sequence of rounds with a particular set of pseudorandom keys an epoch. Intuitively, we would like to claim that if the device passes all the equation tests, then for most epochs and for most rounds within that epoch, the state of the device and its measurements must be (close to) as characterized above: it starts with a qubit initialized to $\ket{+}$, which it measures in the standard basis for the case of a preimage test, and in the Hadamard basis for the case of an equation test. To show this we would like to claim that if the device passes all the equation tests, for most such tests it must produce a valid equation with probability close to $1$. Since each equation test occurs at a random round in the epoch, it should follow from the adaptive hardcore bit property that the sequence of bits that the verifier extracts from the device's answers to preimage tests during that epoch must look statistically random. We give a martingale-based argument to formalize this intuition. 

There is however a bigger challenge to analyzing the protocol --- we must show that the sequence that the verifier extracts from the device's answers to preimage tests must look statistically random even to an infinitely powerful quantum adversary, who may share an arbitrary entangled state with the quantum device. If we could assert that each round of the protocol is played with a qubit exactly in state $\ket{+}$, and measured in the standard basis basis for the case of a preimage test, then this would lead to an easy proof that the extracted sequence looks random to the adversary. Unfortunately the characterization of the device's qubits leaves plenty of room for entanglement with the adversary. Showing that such entanglement cannot leak too much information about the device's measurements was the major challenge in previous work on certified randomness through Bell inequality violations~\cite{VV12,miller2014universal,arnon2018practical}. 
Our cryptographic setting presents a new difficulty, which is that in contrast to the  Bell inequality violation scenarios, in our setting it is not \emph{impossible} for a deterministic device to succeed in the test: it is merely \emph{computationally hard} to do so. This prevents us from directly applying the results in~\cite{miller2014universal,arnon2018practical} and requires us to suitably modify their framework. We describe this part of the argument in more detail below.


In terms of efficiency, 
for the specific LWE-based NTCF  that we construct, our protocol can use as few as $\poly\log(N)$ bits of randomness to 
generate $O(N)$ bits that are statistically within negligible distance from uniform. However, this  requires assuming that the underlying LWE assumption is hard even for sub-exponential size quantum circuits with polynomial-size quantum advice (which is consistent with current knowledge). The more conservative assumption that our variant of LWE is only hard for polynomial size quantum circuits requires $O(N^{\epsilon})$ bits of randomness for generating the NTCF, for any constant $\epsilon >0$. The following is an informal description; see Theorem~\ref{thm:expansion} for a more formal statement.


\begin{theorem}[Informal]
Let $\mathcal{F}$ be an NTCF family and $\lambda$ a security parameter. Let $N = \Omega(\lambda^2)$ and assume the quantum hardness of solving lattice problems of dimension $\lambda$ in time $\poly(N)$. There is an $N$-round protocol for the interaction between a classical polynomial-time verifier and a quantum polynomial-time device such that the protocol can be executed using $\poly(\log(N),\lambda)$ bits of randomness, and for any efficient device and side information $\reg{E}$ correlated with the device's initial state,
$$\Hmin^{\delta}(O|CE)_{\ol{\rho}} \geq  (\xi-o(1)) N\;.$$
Here $\xi$ is a positive constant, $\delta$ is a negligible function of $\lambda$, and $\ol{\rho}$ is the final state of the classical output register $\reg{O}$, the classical register $\reg{C}$ containing the verifier's messages to the device, and the side information $\reg{E}$, restricted to transcripts that are accepted by the verifier in the protocol.
\end{theorem}



\paragraph{Sketch of the security analysis.}
We describe the protocol in slightly more detail (see Section~\ref{sec:protocol} for a formal description). The verifier first uses $\poly(\log(N),\lambda)$ bits of randomness to 
select a pair of functions $\{f_{k,b}\}_{b\in\{0,1\}}$ from an NTCF family, and sends the public function key $k$ to the quantum device. This pair of functions can be interpreted as a single $2$-to-$1$ function $f_k:(b,x)\mapsto f_{k,b}(x)$. The verifier keeps private the trapdoor information that allows to invert $f_k$.
The protocol then proceeds for $N$ rounds. In each round the device first outputs a value $y$ in the common range of $f_{k,0}$ and $f_{k,1}$. After having received $y$, the verifier issues one of two 
challenges: $0$ or $1$, preimage or equation. If the challenge is ``preimage'', then the device must output an $x$ such that $f(x) = y$. If the challenge is 
``equation'' then the device must output a nontrivial binary vector $d$ such that $d\cdot(x_0 \oplus x_1) = 0$, where $x_0$ and $x_1$ are the unique preimages of $y$ under $f_{k,0}$ and $f_{k,1}$ respectively. Since the verifier has the secret key, she can efficiently compute $x_0$ and $x_1$ from $y$, and therefore check the correctness of the
device's response to each challenge. The verifier chooses 
$\poly\log(N)$ rounds in which to issue the challenge $1$, or ``equation'', at random. Selecting these rounds requires only
$\poly\log(N)$ random bits. At the end of each such round, the verifier samples a new pair of functions from the NTCF family, and communicates the new public key to the device. On each of the remaining $N - \poly\log(N)$ rounds the verifier records a bit according to 
whether the device returns the preimage $x_0$, or $x_1$ (e.g.\ recording $0$ for the lexicographically smaller preimage). At the end of the protocol the verifier
uses a strong quantum-proof randomness extractor to extract $\Omega(N)$ bits of randomness from the recorded string (this requires at most an additional $\poly\log(N)$ bits of uniformly random seed).

To guarantee that the extractor produces bits that are statistically close to uniform, we would like to prove that the $N - \poly\log(N)$ random bits recorded by the verifier must have  $\Omega(N)$ bits of (smoothed) min-entropy,\footnote{We refer to Section~\ref{sec:prelim} for definitions of entropic quantities.} even conditioned on the side information available to an infinitely powerful quantum adversary, who may share an arbitrary entangled state with
the quantum device. 

The analysis proceeds as follows. First we assume without loss of generality that the entire protocol is run coherently, i.e.\ we may
assume that the initial state of the quantum device (holding quantum register $\reg{D}$) and the adversary (holding quantum register $\reg{E}$)
is a pure state $\ket{\phi}_\reg{DE}$, since the adversary may as well start with a purification of their joint state. We may also assume that the verifier 
starts with a cat state on $\poly\log(N)$ qubits, and uses one of the registers of the state, $\reg{C}$, to provide the random bits used to select the type of test being performed in each round. (This is for the sake of analysis only, the actual verifier is of course completely classical.) We can similarly  arrange that 
the state remains pure throughout the protocol by using the principle of deferred measurement. Our goal is to show a lower bound on the smooth
min-entropy of the output register $\reg{O}$ in which the verifier has recorded the device's outputs, conditioned on the state $\reg{E}$ of the adversary, and on the register $\reg{C}$ of the cat state  (conditioning on the latter represents the fact that the verifier's choice of challenges may be leaked to the adversary, and we would like security even in this scenario). 
Intuitively, this amounts to bounding the information accessible to the most powerful adversary quantum mechanics allows, conditioned on the joint state of the verifier and device.

In order to bound the entropy of the final state we need to show that the entropy ``accumulates'' at each round of the protocol. A general framework to establish entropy accumulation in quantum protocols such as the one considered here was introduced in~\cite{arnon2018practical}. At a high level, the approach consists in reducing the goal of a min-entropy bound to a bound on the appropriate notion of $(1+\eps)$ quantum conditional R\'enyi entropy, and then arguing that, under suitable conditions on the process that generates the outcomes recorded in the protocol, entropy accumulates sequentially throughout the protocol.

In a little more detail, the first step on getting a handle on the smooth min-entropy is to use the quantum asymptotic equipartion property (QAEP)~\cite{tomamichel2009fully} to relate it to the $(1+\eps)$ conditional R\'enyi entropy, for suitably small $\eps$. The second step uses a duality relation for the conditional R\'enyi entropy to relate the $(1+\eps)$ conditional R\'enyi entropy of the output register $\reg{O}$, conditioned on the adversary side information in $\reg{R}$ and the register $\reg{C}$ of the cat state,  to a quantity analogous to the $(1-\eps')$ conditional R\'enyi entropy of the output register, conditioned on the register $\reg{E}$ for the device, and a purifying copy of the register $\reg{C}$ of the cat state. The latter quantity, a suitable conditional entropy of the output register conditioned on the challenge register and the state of the device, is the quantity that we ultimately aim to bound. Note what these transformations have achieved for us: it is now sufficient to consider as side information only ``known'' quantities in the protocol, the verifier's choice of challenges and the device's state; the information held by the adversary plays no other role than that of a purifying register. 

As mentioned earlier, our cryptographic setting presents the additional difficulty that our guarantee is only that it is {computationally hard} for a deterministic device to succeed in the protocol. The results in~\cite{arnon2018practical,miller2014universal} crucially rely on the fact that the process that generates the randomness does so irrespective of the quantum state in which it is initialized (as long as the output of the process satisfies the test's success criterion). This requirement comes  from the conditioning that is performed in order to show that entropy accumulates; in our setting, conditioning is more delicate as it can in principle induce non-computationally efficient states for the device. 



Recall that we argued that for a single round of the protocol, we can decompose the device's Hilbert space into a direct sum of one- or two-dimensional subspaces, such that within most two-dimensional subspace the ``preimage'' and ``equation'' measurements correspond to orthonormal bases that make an angle close to $\pi/4$ with each other.
Showing that the R\'enyi entropy accumulates in each round requires a device in which \emph{all} angles are close to $\pi/4$, not ``almost all''. To accommodate for this we ``split'' the state of the device into its component on the good subspace, where the angles are unbiased, and the bad subspace, where the measurements may be aligned. The fact that the distinction between good and bad subspace is not measured in the protocol, but is only a distinction made for the analysis, requires us to apply a fairly delicate martingale based argument that takes into account possible interference effects and bounds those ``branches'' where the state has gone through the bad subspace an improbably large number of times. Whenever the state lies in the good susbpace, we can appeal to
an uncertainty principle from~\cite{miller2014universal} to show that the device's measurement increases the conditional R\'enyi entropy of the output register by a small additive constant. 
Pursuing this approach across all $N$ rounds, we obtain a linear lower bound on the conditional R\'enyi entropy of the output register, conditioned on the  state of the device. As argued above this in turn translates into a linear lower bound on the smooth conditional min-entropy of the output, conditioned on the state of the adversary and the verifier's choice of challenges. It only remains to apply a quantum-proof randomness extractor to the output, using a poly-logarithmic number of additional bits of randomness, to obtain the final result. 


\paragraph{Our NTCF Family.} Our goal is to construct a family of pairs of injective functions $f_0, f_1$ with the same image such that it is hard to find a collision $x_0, x_1$ with $f_0(x_0)=f_1(x_1)$, but so that given a suitable trapdoor it is possible to recover, for any $y$, values $x_0, x_1$ such that $f_0(x_0)=f_1(x_1)=y$. We do this by relying on the hardness of the Learning with Errors (LWE) problem \cite{regev2005}. LWE states that given a public uniformly random matrix $\mx{A}\in\bbZ_q^{m \times n}$ for $m \gg n$, it is intractable to distinguish between $\vc{u}=\mx{A}\vc{s}+\vc{e}\pmod{q}$ and a uniform vector, for a uniform vector $\vc{s}$ and small discrete Gaussian vector $\vc{e}$ (all arithmetic from here on is performed modulo $q$; we use $\oplus$ to denote binary XOR). Inspired by \cite{mahadev2017classicalv1}, our function pair will be characterized by $(\mx{A},\vc{u}=\mx{A}\vc{s}+\vc{e})$, but for a \emph{binary} vector $\vc{s}$.\footnote{It is known that LWE is hard even with binary secrets. We do not use this property explicitly but rather employ the respective techniques in our proof.} The trapdoor for our function is a {lattice trapdoor} for $\mx{A}$ that allows to recover $\vc{s}, \vc{e}$ given a vector of the form $\mx{A}\vc{s}+\vc{e}$ (it is possible to generate $\mx{A}$ together with a trapdoor such that $\mx{A}$ is indistinguishable from uniform, as originally shown by Ajtai \cite{ajtai99}).

%A natural choice would have been to define $f_b(\vc{x})=\mx{A}\vc{x}+b\cdot\vc{u}$. Such a shift would be hard to detect, but unfortunately the images of $f_0, f_1$ are disjoint. If we wanted the images to be identical, we could have instead defined $f_b(\vc{x})=\mx{A}\vc{x}+b\cdot(\mx{A}\vc{s})$, which would easily guarantee that the two functions are injective and have the same image. Alas, the latter definition is not efficiently computable given $\mx{A}, \vc{u}$. To reconcile the two approaches,
The structure of the LWE problem motivates us to consider functions $f_0$, $f_1$ that range over probability distributions. Specifically, we define the distribution $f_b(\vc{x})$ as $f_b(\vc{x})=\mx{A}\vc{x}+b\cdot(\mx{A}\vc{s})+\vc{e}'$ where $\vc{e}'$ is a discrete Gaussian random variable with a sufficiently wide Gaussian parameter. Observe that the functions have overlapping images in the following sense: $f_0(\vc{x}) = f_1(\vc{x-s})$. Moreover, since $\mx{A}\vc{s}+\vc{e}'$ is statistically indistinguishable from $\vc{u}+\vc{e}'$, we can efficiently sample from the distribution $f_b(\vc{x})$ up to negligible statistical distance.

This probabilistic notion complicates the definition and use of the family, but the principles are similar to the deterministic version.\footnote{Another possible variant is to define $f_b(\vc{x})=\lfloor\mx{A}\vc{x}+b\cdot(\mx{A}\vc{s})\rceil$ where $\lfloor \cdot \rceil$ is a rounding function that truncates ``many'' of the least significant bits of its operand. However, we remain with the Gaussian variant which is easier to analyze.}

\def\hatd{\hat{d}}

\paragraph{Adaptive Hardcore Bit.}

Finally, we need to show the adaptive hardcore bit property. Formally, letting $\vc{x}_0, \vc{x}_1 \in \bbZ_q^n$ be a collision, and letting $z_0, z_1 \in \{0,1\}^{n \log q}$ be their binary representations, respectively, we need to show that it is intractable to come up with a pair $(b,z_b)$, for some $b\in\{0,1\}$, together with a nontrivial vector $d$ and with the value $d \cdot (z_0 \oplus z_1)$, with probability noticeably better than $\frac{1}{2}$. ``Nontrivial'' here means belonging to a well defined and efficiently recognizable set $D$ with density $\approx 1$ in $\{0,1\}^{n \log q}$ (e.g.\ the zero vector is obviously excluded). Assume for the sake of this overview that we get a tuple $(z_0, d, c)$. We first notice that since $\vc{x}_0, \vc{x}_1$ is a collision, then $\vc{x}_1 = \vc{x}_0 - \vc{s}\pmod{q}$. We now use the fact that $\vc{s}$ is a binary vector to show, using simple arithmetic, that $z_0 \oplus z_1$ can be expressed as a linear function of the bits of $\vc{s}$, so that $d \cdot (z_0 \oplus z_1) = \hatd \cdot \vc{s}\pmod{2}$, for some $\hatd\in\{0,1\}^n$.  (The description of this transformation will effect our choice of the set $D$.) We thus need to show that it is intractable, given the instance $(\mx{A},\vc{u}=\mx{A}\vc{s}+\vc{e})$, to come up with $\hatd, \hatd \cdot \vc{s}\pmod{2}$. To prove this we use the lossiness technique used in \cite{GKPV10} and show that this is equivalent to coming up with $\hatd, \hatd \cdot \vc{s}\pmod{2}$ given $\mx{B}, \mx{B}\vc{s}$ where $\mx{B} \in \bbZ_q^{k \times n}$ is now a highly shrinking function, even for binary inputs, i.e.\ $k\log q \ll n$. This seems like an easy task since the adversary now doesn't have the complete information about $\vc{s}$ so it shouldn't be able to compute $\hatd \cdot \vc{s}\pmod{2}$ for any reasonable $\hatd$, except $\hatd$ might depend on $\mx{B}$ itself (recall that $\hatd$ is chosen adversarially). We prove via Fourier analysis that if $\mx{B}$ is sufficiently shrinking, then there is no $\hatd$ that can take advantage of the dependence on $\mx{B}$, which completes the proof.


\paragraph{Concurrent and related work.}
The idea of using a TCF as a basic primitive in interactions between an efficient quantum prover and a classical verifier has been 
further developed in recent work by Mahadev \cite{mahadev2017classical}, giving the first construction of a quantum fully homomorphic encryption scheme with classical keys. 
In further follow-up work, Mahadev~\cite{UrmilaVerifiability} shows a remarkable use of a NTCF family with adaptive hardcore bit. Namely, that the NTCF can be used to certify that a prover measures a qubit in a prescribed basis (standard or Hadamard). This allows to achieve single prover \emph{verifiability} for quantum computations using a purely classical verifier (but relying on computational assumptions).

Independently of this work, a construction of trapdoor one-way functions with second preimage resistance based on LWE was recently introduced in~\cite{cojocaru2018delegated}, where it is used to achieve delegated computation in the weaker honest-but-curious model for the adversary (i.e.\ without soundness against provers not following the protocol). The family of functions considered in~\cite{cojocaru2018delegated} is not sufficient for our purposes, as it lacks the  adaptive hardcore bit property.

After the completion of our work, in~\cite{gheorghiu2019computationally} the construction of NTCF family introduced here was extended to a more general hardcore bit property (informally, over $\Z_8$ instead of $\Z_2$ here) and used to implement a two-party functionality called ``remote state preparation'' by which a classical client can ``force'' the preparation of one out of eight possible single-qubit quantum states by the prover. The authors of~\cite{cojocaru2019qfactory} also generalize~\cite{cojocaru2018delegated} to obtain a similar functionality; however, their construction does not offer the property of being verifiable (informally, it is possible for the server to prepare a state that is not the expected one). 

We believe that the technique of constraining the power of a quantum device using NTCFs promises to be a powerful tool for the field of untrusted quantum devices. %applications where a single quantum machine is to be forced to perform a certain operation in a prescribed manner.



\paragraph{Organization.} We start with some notation and preliminaries in Section~\ref{sec:prelim}. Section~\ref{sec:tcf} contains the definition of a noisy trapdoor claw-free family (NTCF). Our construction for such a family is given in Section~\ref{sec:lwetcf} (with Appendix~\ref{sec:lweprelim} containing relevant preliminaries on the learning with errors problem). The randomness generation protocol is described in Section~\ref{sec:protocol}. In Section~\ref{sec:device} we introduce our formalism for modeling the actions of an arbitrary prover, or device, in the protocol. In Section~\ref{sec:soundness} we analyze a single round of the protocol, and in Section~\ref{sec:multi-round} we show that randomness accumulates across multiple rounds. 



\paragraph{Acknowledgments.}
We thank Tony Metger and the anonymous JACM referees for corrections and suggestions that improved the presentation of the paper. 
Zvika Brakerski is supported by the Israel Science Foundation (Grant No.\ 468/14), Binational Science Foundation (Grants No.\ 2016726, 2014276), and by the European Union Horizon 2020 Research and Innovation Program via ERC Project REACT (Grant 756482) and via Project PROMETHEUS (Grant 780701). Paul Christiano and Urmila Mahadev are supported by a Templeton Foundation Grant 52536, ARO Grant W911NF-12-1-0541, and NSF Grant CCF-1410022.
Umesh Vazirani is supported by Templeton Foundation Grant 52536, ARO Grant W911NF-12-1-0541, NSF Grant CCF-1410022, MURI Grant FA9550-18-1-0161 and a Vannevar Bush Faculty Fellowship.
Thomas Vidick is supported by NSF CAREER Grant CCF-1553477, AFOSR YIP award number FA9550-16-1-0495, MURI Grant FA9550-18-1-0161, a CIFAR Azrieli Global Scholar award, and the IQIM, an NSF Physics Frontiers Center (NSF Grant PHY-1125565) with support of the Gordon and Betty Moore Foundation (GBMF-12500028).
 


==> lweprelim.tex <==

In this section we give some background on the Learning with Errors problem (LWE). 
For a positive real $B$ and positive integers $q$, the truncated discrete Gaussian distribution over $\mZ_q$ with parameter $B$ is supported on $\{x\in\mZ_q:\,\|x\|\leq B\}$ and has density
\begin{equation}\label{eq:d-bounded-def}
 D_{\mZ_q,B}(x) \,=\, \frac{e^{\frac{-\pi\lVert x\rVert^2}{B^2}}}{\sum\limits_{x\in\mZ_q,\, \|x\|\leq B}e^{\frac{-\pi\lVert x\rVert^2}{B^2}}} \;.
\end{equation}
We note that for any $B>0$, the truncated and non-truncated distributions have statistical distance that is exponentially small in $B$~\cite[Lemma 1.5]{banaszczyk1993new}. For a positive integer $m$, the truncated discrete Gaussian distribution over $\mZ_q^m$ with parameter $B$ is supported on $\{x\in\mZ_q^m:\,\|x\|\leq B\sqrt{m}\}$ and has density
\begin{equation}\label{eq:d-bounded-def-m}
\forall x = (x_1,\ldots,x_m) \in \mZ_q^m\;,\qquad D_{\mZ_q^m,B}(x) \,=\, D_{\mZ_q,B}(x_1)\cdots D_{\mZ_q,B}(x_m)\;.
\end{equation}

\begin{lemma}\label{lem:distributiondistance}
Let $B$ be a positive real number and $q,m$ be positive integers. Let $\*e \in \mZ_q^m$. The Hellinger distance between the distribution $D = D_{\mZ_q^{m},B}$ and the shifted distribution $D+\*e$ satisfies
\begin{equation}
H^2(D,D+\*e) \,\leq\, 1- e^{\frac{-2\pi \sqrt{m}\|\*e\|}{B}}\;,
\end{equation}
and the statistical distance between the two distributions satisfies
\begin{equation}
\big\| D - (D+\*e) \big\|_{TV}^2 \,\leq\, 2\Big(1 - e^{\frac{-2\pi \sqrt{m}\|\*e\|}{B}}\Big)\;.
\end{equation}
\end{lemma}

\begin{proof}
Let $\tau = \sum\limits_{x\in\mZ_q,\, \|x\|\leq B}e^{\frac{-\pi\lVert x\rVert^2}{B^2}}$. We can compute
\begin{eqnarray*}
\sum_{\*e_0\in \mZ_q^m} \sqrt{D_{\mZ_q^{m},B}(\*e_0)D_{\mZ_q^{m},B}(\*e_0-\*e)} &=& \sum_{\*e_0\in \mZ_q^m}  \sqrt{D_{B}(\*e)D_{B}(\*e_0-\*e)}\\
&=& \frac{1}{\tau^m}\sum_{\*e\in \mZ_q^m}e^{\frac{-\pi(\|\*e_0\|^2 + \|\*e_0 - \*e\|^2)}{2B^2}}\\
&\geq& \frac{1}{\tau^m}\sum_{\*e_0\in \mZ_q^m}e^{\frac{-\pi(\|\*e_0\|^2 + (\|\*e_0\| + \|\*e\|)^2)}{2B^2}}\\
&=& \frac{1}{\tau^m}\sum_{\*e_0\in \mZ_q^m}e^{\frac{-\pi(\|\*e_0\|^2)}{B^2}}e^{\frac{-\pi(2\|\*e_0\|\|\*e\|)}{2B^2}}e^{\frac{-\pi(\|\*e\|^2)}{2B^2}}\\
&\geq& e^{\frac{-\pi(\|\*e\|^2 + 2\|\*e_0\|\|\*e\|)}{2B^2}}\frac{1}{\tau^m}\sum_{\*e_0\in \mZ_q^m}e^{\frac{-\pi(\|\*e_0\|)^2}{B^2}}\\
&=& e^{\frac{-\pi(\|\*e\|^2 + 2\|\*e_0\|\|\*e\|)}{2B^2}}\label{eq:distequality}\\
&\geq& e^{\frac{-2\pi \|\*e_0\|\|\*e\|}{B^2}}\;.
\end{eqnarray*}
Using the fact that for any $\*e_0$ in the support of $D_{\mZ_q^m,B}$, $\|\*e_0\|\leq B\sqrt{m}$,  gives the claimed bound.
\end{proof}



\begin{definition}\label{def:lwe-ass}
For a security parameter $\lambda$, let $n,m,q\in \bbN$ be integer functions of $\lambda$. Let $\chi = \chi(\lambda)$ be a distribution over $\mZ$. The $\lwe_{n,m,q,\chi}$ problem is to distinguish between the distributions $(\*A, \*A\*s + \*e \pmod{q})$ and $(\*A, \*u)$, where $\*A$ is uniformly random in $\bbZ_q^{n \times m}$, $\*s$ is a uniformly random row vector in $\mZ_q^n$, $\vc{e}$ is a  row vector drawn at random from the distribution $\chi^m$, and $\*u$ is a uniformly random vector in $\mZ_q^m$. Often we consider the hardness of solving $\lwe$ for {any} function $m$ such that $m$ is at most a polynomial in $n \log q$. This problem is denoted $\lwe_{n,q,\chi}$. In this paper we make the assumption that no quantum polynomial-time procedure can solve the $\lwe_{n,q,\chi}$ problem with more than a negligible advantage in $\lambda$, even when given access to a quantum polynomial-size state depending on the parameters $n,m,q$ and $\chi$ of the problem. We refer to this assumption as ``the $\lwe_{n,q,\chi}$ assumption''.
\end{definition}



As shown in \cite{regev2005,PRS17}, for any $\alpha>0$ such that  $\sigma = \alpha q \ge 2 \sqrt{n}$ the $\lwe_{n,q,D_{\mZ_q,\sigma}}$ problem,  where $D_{\mZ_q,\sigma}$ is the discrete Gaussian distribution, is at least as hard as approximating the shortest independent vector problem ($\sivp$) to within a factor of $\gamma = \otild({n}/\alpha)$ in \emph{worst case} dimension $n$ lattices. This is proven using a quantum reduction. Classical reductions (to a slightly different problem) exist as well \cite{Peikert09,BLPRS13} but with somewhat worse parameters. The best known (classical or quantum) algorithm for these problems run in time $2^{\otild(n/\log \gamma)}$. For our construction we assume hardness of the problem against a quantum polynomial-time adversary in the case that $\gamma$ is a super polynomial function in $n$. This is a commonly used assumption in cryptography (for e.g. homomorphic encryption schemes such as \cite{fhelwe}).





We use two additional properties of the LWE problem. The first is that it is possible to generate LWE samples $(\*A,\*A\*s+\*e)$ such that there is a trapdoor allowing recovery of $\*s$ from the samples. 

\begin{theorem}[Theorem 5.1 in~\cite{miccancio2012}]\label{thm:trapdoor}
Let $n,m\geq 1$ and $q\geq 2$ be such that $m = \Omega(n\log q)$. There is an efficient randomized algorithm $\GenTrap(1^n,1^m,q)$ that returns a matrix $\*A \in \mZ_q^{m\times n}$ and a trapdoor $t_{\*A}$ such that the distribution of $\*A$ is negligibly (in $n$) close to the uniform distribution. Moreover, there is an efficient algorithm $\Invert$ that, on input $\*A, t_{\*A}$ and $\*A\*s+\*e$ where $\|\*e\| \leq q/(C_T\sqrt{n\log q})$ and $C_T$ is a universal constant, returns $\*s$ and $\*e$ with overwhelming probability over $(\*A,t_{\*A})\leftarrow \GenTrap$. \end{theorem}

The second property is the existence of a ``lossy mode'' for LWE. The following definition is Definition~3.1 in~\cite{lwr}. 

\begin{definition}\label{def:lossy}
Let $\chi = \chi(\lambda)$ be an efficiently sampleable distribution over $\mZ_q$. Define a lossy sampler $\tilde{\*A} \leftarrow \lossy(1^n,1^m,1^\ell,q,\chi)$ by  $\tilde{\*A} = \*B\*C +\*F$, where $\*B\leftarrow_U \mZ_q^{m\times \ell}$, $\*C\leftarrow_U \mZ_q^{\ell \times n}$, $\*F\leftarrow \chi^{m\times n}$. 
\end{definition}

\begin{theorem}[Lemma 3.2 in~\cite{lwr}]\label{thm:lossy}
Under the $\lwe_{\ell,q,\chi}$ assumption, the distribution of $\tilde{\*A} \leftarrow \lossy(1^n,1^m,1^\ell,q,\chi)$ is computationally indistinguishable from $\*A\leftarrow_U \mZ_q^{m\times n}$. 
\end{theorem}


